Magnetars From Magnetized Cores Created by a Strong Interaction Phase Transition

We consider a model where the strong magnetic fields of magnetars arise from a high baryon density, magnetized core. In this framework magnetars are distinguished from pulsars by their higher masses and central density. For magnetars, as core densities exceed a threshold, the strong interaction induces a phase transition to a neutral pion condensate that aligns all magnetic moments. The core magnetic field is initially shielded by the ambient high conductivity plasma. With time the shielding currents dissipate transporting the core field out, first to the crust and then breaking through the crust to the surface of the star. Recent observations provide strong support for this model which accounts for several properties of magnetars and also enables us to identify new magnetars.

==> scibiblio <==
\begin{thebibliography}{99}
\bibitem{palmer+05} D.M. Palmer\textit{ et al., 
   Nature }{\bf 434}, 1107 (2005)
\bibitem{hurley+05} K. Hurley \textit{et al.,
   Nature} {\bf 434}, 1098 (2005)
\bibitem{duncan+thompson92} R.C. Duncan, C. Thompson,
   \textit{Astrophys. J.} {\bf 392}, L9 (1992)
\bibitem{thompson+duncan95} C. Thompson, R.C. Duncan,
   \textit{Mon. Not. R. Astron. Soc. }{\bf 275}, 255 (1995)
\bibitem{thompson+02} C. Thompson, M. Lyutikov, S.R. Kulkarni,
   \textit{Astrophys. J.} {\bf 574}, 332 (2002) 
\bibitem{leahy0} D.Leahy, R. Ouyed, http:/arXiv.org/abs/arXiv:0710.2114v2 (2007)
\bibitem{wickramasinghe}L. Ferrario, D. Wickramasinghe, \textit{Mon. Not. R. Astron. Soc.} {\bf367},1323(2006)
\bibitem{gaensler0} B. M. Gaensler \textit{et al, Astrophys. J.} {\bf620}, L95 (2005)
\bibitem{muno0}M.P. Muno, AIP Conf. Proc. {\bf924},166 (2007)
\bibitem{vink0} J. Vink, L. Kuiper,  \textit{Mon. Not. R. Astron. Soc.} {\bf370}, L14 (2006)
\bibitem{heger0} A. Heger, S.E. Woosley, H. C. Spruit, \textit{Astrophys. J.} {\bf626}, 350 (2005) 
\bibitem{ddarxiv}A. Dar, A.De Rujula, http:/arXiv.org/abs/astro-ph/0002014v2(2000)
\bibitem{ddgreco} A. Dar, A.De Rujula, in \textit{Results and Perspectives in Particle Physics }, Mario Greco Ed.            {\bf Vol. 17}, 13 (2000) 
\bibitem{dar1999a} A. Dar, \textit{A\&A Suppl. }{\bf138}, 505 ,(1999)
\bibitem{marsden0} D. Marsden, R. E. Rothschild, R.E. Lingenfelter, \textit{Astrophys. J.} {\bf520}, L107 (1999).
\bibitem{dbvsarxiv} D. Bhattacharya and V. Soni, http://arXiv.org/abs/0705.0592:v2 (2007)
\bibitem{woltjer64} L. Woltjer, 
  \textit{ Astrophys. J.} {\bf 140}, 1309 (1964)
\bibitem{dbvsplb} V. Soni, D. Bhattacharya, \textit{Phys. Lett. B} {\bf643}, 158 (2006)
\bibitem{dbvshepph} V. Soni, D. Bhattacharya, http://arXiv.org/abs/ hep-ph/0504041 (2005)
\bibitem{goldreisenegger92} P. Goldreich, A. Reisenegger, 
   \textit{Astrophys. J.} {\bf 395}, 250 (1992)
\bibitem{spitzer78} L. Spitzer, \textit{Physical Processes in the Interstellar
   Medium,} John Wiley \& Sons, New York (1978)
\bibitem{dautry} F. Dautry, E.M. Nyman, 
   \textit{Nucl. Phys.A} {\bf A319} 323 (1979)
\bibitem{kutschera+90} M. Kutschera, W. Broniowski, A. Kotlorz,
   \textit{Nucl. Phys.A}{\bf A516}, 566 (1990)
\bibitem{kaminker} A.D. Kaminker et al,  
    \textit{ Mon. Not. Roy. Astron. Soc.} {\bf 371}, 477 (2006)
\bibitem{ruderman91} M. Ruderman,
   \textit{Astrophys. J.} {\bf 366}, 291 (1991)
\bibitem{kaspiarxiv} M.A. Livingstone, V. M. Kaspi, F. P Gavrill, http:/arXiv.org/abs/astro-ph/ 0905.3567v2 (2010).
\bibitem{zhang+lin05} S.N. Zhang, J. Lin, talk presented at the 
   Urunci meeting on Radio pulsars (2005)
\bibitem{kaminker07} A.D. Kaminker et al , 
    \textit{Astrophys Space Sci.} {\bf 308}, 423 (2007).
\bibitem{woods1999a} P. M. Woods, \textit{et al., Astrophys. J.} {\bf524}, L55 (1999)

\bibitem{gavrill0} F. P. Gavrill \textit{et al, Science} {\bf319}, 1802( 2008).

\bibitem{alpar_pines_shaham} M. Ali Alpar, K.S. Cheng, D. Pines and J. Shaham, \textit{Mon. Not. R. Astr. Soc.} 
{\bf 233}, 25 (1998) .
\bibitem{lyne} A.G. Lyne, \textit{Nature} {\bf 326}, 569 (1987).
\bibitem{alpar_vela} M.A. Alpar, \textit{Adv. Space Res. }{\bf Vol 21, No. 1/2}, 159 (1998).
\bibitem{gonzalez0} M. E. Gonzalez, V. M. Kaspi, A.G. Lyne, M.J. Pivovaroff \textit{ Astrophys. J.} {\bf610}, L37(2004).
\end{thebibliography}

